Solving Large Multicommodity Network Flow Problems on GPUs

We consider the all-pairs multicommodity network flow problem on a network with capacitated edges. The usual treatment keeps track of a separate flow for each source-destination pair on each edge; we rely on a more efficient formulation in which flows with the same destination are aggregated, reducing the number of variables by a factor equal to the size of the network. Problems with hundreds of nodes, with a total number of variables on the order of a million, can be solved using standard generic interior-point methods on CPUs; we focus on GPU-compatible algorithms that can solve such problems much faster, and in addition scale to much larger problems, with up to a billion variables. Our method relies on the primal-dual hybrid gradient algorithm, and exploits several specific features of the problem for efficient GPU computation. Numerical experiments show that our primal-dual multicommodity network flow method accelerates state of the art generic commercial solvers by $100\times$ to $1000\times$, and scales to problems that are much larger. We provide an open source implementation of our method.

==> formatting.tex <==
% Fonts.
%\usefonttheme{serif}
%\usepackage{palatino}
% \usepackage{mathpazo}
% \usepackage{eulervm}
%\usepackage[T1]{fontenc}

% Template changes.
\let\oldsection\section
\renewcommand{\section}[1]{\oldsection{#1}
\begin{frame}
    \frametitle{Outline}
    \tableofcontents[currentsection,currentsubsection]
\end{frame}
}

\setbeamertemplate{navigation symbols}{}
\setbeamersize{text margin left=1.2cm, text margin right=1.2cm}
\usecolortheme[rgb={0.6,0,0}]{structure}

\setbeamertemplate{frametitle} {
  \vskip 0.65cm
  \hskip -0.4cm
  {\large\bf \insertframetitle}
}

\setbeamertemplate{itemize items}[default]

\setlength{\parskip}{4pt}

\newcommand\footlineon{
  \setbeamertemplate{footline} {
    \begin{beamercolorbox}[ht=2.5ex,dp=1.125ex,leftskip=.8cm,rightskip=.6cm]{structure}
      \footnotesize \insertsection
      \hfill
      {\insertframenumber}
    \end{beamercolorbox}
    \vskip 0.45cm
  }
}
\footlineon

% \newcounter{algorithmctr}[section]
% \renewcommand{\thealgorithmctr}{\thesection.\arabic{algorithmctr}}

